Serverless Scheduling Policies based on Cost Analysis

Current proprietary and open-source serverless platforms follow opinionated, hardcoded scheduling policies to deploy the functions to be executed over the available workers. Such policies may decrease the performance and the security of the application due to locality issues (e.g., functions executed by workers far from the databases to be accessed). These limitations are partially overcome by the adoption of APP, a new platform-agnostic declarative language that allows serverless platforms to support multiple scheduling logics. Defining the "right" scheduling policy in APP is far from being a trivial task since it often requires rounds of refinement involving knowledge of the underlying infrastructure, guesswork, and empirical testing. In this paper, we start investigating how information derived from static analysis could be incorporated into APP scheduling function policies to help users select the best-performing workers at function allocation. We substantiate our proposal by presenting a pipeline able to extract cost equations from functions' code, synthesising cost expressions through the usage of off-the-shelf solvers, and extending APP allocation policies to consider this information.

==> capp_figure.tex <==

\begin{adjustbox}{width=\textwidth}
 \noindent\begin{tikzpicture}
 \node[draw,text height= 1.4cm, text depth=.8cm, minimum width=5.3cm] (app) at (5,0) {
 \hspace{-.5em}\begin{lstlisting}[linewidth=5.2cm,language=yaml,backgroundcolor=\color{Gray!10},mathescape=true]
 - premUser:
   - $\hl{workers}$: 
       - $\hl{wrk}$: W1
       - $\hl{wrk}$: W2
     $\hl{strategy}$: $\hlopt{min\_latency}$
 \end{lstlisting}};
 \node[above] at (app.north) {Abstract Cost-aware \APP{} script};
 
 \node[draw, text height=1cm, text depth=.4cm] (static) at (0,-3) {
 \hspace{-.2em}\begin{lstlisting}[linewidth=5.2cm,language=JavaScript,mathescape=true,numbers=none]
 // tag: premUser
 ( isPremiumUser, par ) => {
   ...
 }
 \end{lstlisting}
 };
 \node[right] at (static.east) {Listing~\ref{lst.if_internal}};
 
 \node[draw, text height=1cm, text depth=.4cm, minimum width=5.3cm] (dynamic) at (10,-3) {
 \hspace{-2.5em}\begin{lstlisting}[linewidth=5.2cm,language=JavaScript,mathescape=true,numbers=none]
 // tag: premUser
 ( username, par ) => {
   ...
 }
 \end{lstlisting}
 };
 \node[left] at (dynamic.west) {Listing~\ref{lst.if_external}};
   
 \draw[-stealth, line width=1pt] (app.south west) -- (static.north) node[midway, left] {Request for\phantom{A}};
 \draw[-stealth, line width=1pt] (app.south east) -- (dynamic.north) node[midway, right] {\hspace{1em} Request for};
 
 \node[draw, align=right, text height=1cm, text depth=.85cm, minimum width=8cm] (eqStatic) at (0, -6.45) {
 \hspace{-6cm}\begin{lstlisting}[linewidth=7.9cm,language=CostExp,mathescape=true]
 eq( ... ).
 eq( ... ).
 \end{lstlisting}
 };
 \node[draw,text height=1.25cm, text depth=.85cm, minimum width=8cm] (eqDynamic) at (10, -6.45) {
 \hspace{-6cm}\begin{lstlisting}[linewidth=7.9cm,language=CostExp,mathescape=true]
 eq( ... ).
 eq( ... ).
 \end{lstlisting}
 };
 
 \draw[-stealth, line width=1pt] (static.south) -- (eqStatic.north) node[midway, left] {Inferred Cost Equations};
 \draw[-stealth, line width=1pt] (dynamic.south) -- (eqDynamic.north) node[midway, right] {Inferred Cost Equations};
 
 
 \node[draw,text height=1.25cm, text depth=.85cm, minimum width=8cm] (appStatic) at (0, -10.45) {
 \hspace{-.2em}\begin{adjustbox}{width=9.5cm}
 \begin{lstlisting}[linewidth=.85\textwidth,language=yaml,backgroundcolor=\color{Gray!10},mathescape=true]
 - $\hl{workers}$: 
     - $\hl{wrk}$: W1
     - $\hl{wrk}$: W2
   $\hl{strategy}$: 
     W $\hl{where}$ $\hl{min}$( W.$\hl{latency}$( PremiumService ) ) [ isPremium ],
            $\hl{min}$( W.$\hl{latency}$( BasicService ) )   [ $\neg$isPremium ]
 \end{lstlisting}
 \end{adjustbox}
 };
 \node[below] at (appStatic.south) {Concrete Cost-aware \APP{} script};
 
 \node[draw,text height=1.4cm, text depth=1cm, minimum width=8.2cm] (appDynamic) at (10, -10.3) {
 \hspace{-.5em}\begin{adjustbox}{width=8cm}
 \begin{lstlisting}[linewidth=.69\textwidth,language=yaml,backgroundcolor=\color{Gray!10},mathescape=true]
 - $\hl{workers}$: 
     - $\hl{wrk}$: W1
     - $\hl{wrk}$: W2
   $\hl{strategy}$:
     W $\hl{where}$ $\hl{min}$( W.$\hl{latency}$( isPremiumUser )
               + $\hl{max}$( W.$\hl{latency}$(PremiumService), 
                      W.$\hl{latency}$(BasicService) ) )
 \end{lstlisting}
 \end{adjustbox}
 };
 \node[below] at (appDynamic.south) {Concrete Cost-aware \APP{} script};
 
 \draw[-stealth, line width=1pt] (eqStatic.south) -- (appStatic.north) node[midway, left] {Computed \APP{} Script};
 \draw[-stealth, line width=1pt] (eqDynamic.south) -- (appDynamic.north) node[midway, right] {Computed \APP{} Script};
   
 \end{tikzpicture}
 \end{adjustbox}

==> eptcsdata.tex <==
\providecommand{\firstpage}{40}
\providecommand{\publicationstatus}{Maurice H. ter Beek and Clemens Dubslaff (Eds.):\\ Proceedings of the First Workshop on Trends\\
in Configurable Systems Analysis (TiCSA'23)\\
EPTCS 392, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.392.3}{10.4204/EPTCS.392.3}}

